Compositional Generalization for Data-to-Text Generation

Data-to-text generation involves transforming structured data, often represented as predicate-argument tuples, into coherent textual descriptions. Despite recent advances, systems still struggle when confronted with unseen combinations of predicates, producing unfaithful descriptions (e.g. hallucinations or omissions). We refer to this issue as compositional generalisation, and it encouraged us to create a benchmark for assessing the performance of different approaches on this specific problem. Furthermore, we propose a novel model that addresses compositional generalization by clustering predicates into groups. Our model generates text in a sentence-by-sentence manner, relying on one cluster of predicates at a time. This approach significantly outperforms T5~baselines across all evaluation metrics.Notably, it achieved a 31% improvement over T5 in terms of a metric focused on maintaining faithfulness to the input.

==> Sections/Backup.tex <==
\section{Taylor Expension for the Marginal Likelihood}\label{sec:appendix_taylor}

Here we show a detailed explanation of \autoref{Eq:8}. First, we do the first-order Taylor expansion of the likelihood function $p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right )$ at the expectation $\mathbb{E}_{\textbf{C}\sim p\left ( \textbf{C} | \textbf{X} \right )} \textbf{C}$, i.e. $\bar{\mathbf{C}}$:

\begin{equation}\label{Eq:Append_1}
\begin{split}
p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) \approx p\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) + p'\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) \left ( \textbf{C} - \bar{\textbf{C}} \right )
\end{split}
\end{equation}
Then the marginal distribution of $\textbf{Y}$ can be written as:
\begin{equation}\label{Eq:Append_2}
\begin{split}
\mathbb{E}_{\textbf{C}\sim p\left ( \textbf{C} | \textbf{X} \right )} p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) & \approx \mathbb{E}_{\textbf{C}\sim p\left ( \textbf{C} | \textbf{X} \right )} \left [ p\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) + p'\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) \left ( \textbf{C} - \bar{\textbf{C}} \right ) \right ] \\
& = \mathbb{E}_{\textbf{C}\sim p\left ( \textbf{C} | \textbf{X} \right )} p\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) + \mathbb{E}_{\textbf{C}\sim p\left ( \textbf{C} | \textbf{X} \right )} p'\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) \left ( \textbf{C} - \bar{\textbf{C}} \right ) \\
& = p\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) + p'\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) \mathbb{E}_{\textbf{C}\sim p\left ( \textbf{C} | \textbf{X} \right )}  \left ( \textbf{C} - \bar{\textbf{C}} \right )
\end{split}
\end{equation}
Since $\mathbb{E}_{\textbf{C}\sim p\left ( \textbf{C} | \textbf{X} \right )}  \left ( \textbf{C} - \bar{\textbf{C}} \right )$ is $0$, in the end, we have:
\begin{equation}\label{Eq:Append_3}
\mathbb{E}_{\textbf{C}\sim p\left ( \textbf{C} | \textbf{X} \right )} p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) \approx p\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) 
\end{equation}
Thus,
\begin{equation}\label{Eq:Append_4}
\log \mathbb{E}_{\textbf{C}\sim p\left ( \textbf{C} | \textbf{X} \right )} p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) \approx \log p\left ( \textbf{Y} | \bar{\textbf{C}}, \textbf{X} \right ) 
\end{equation}

\section{Transformer-based Weight Predication}\label{sec:appendix_rl}
Here we show detailed derivation of \autoref{Eq:11}.
\begin{equation}\label{Eq:Append_5}
\begin{split}
\bigtriangledown_{\phi } \mathbb{E}_{\textbf{C}\sim p_{\phi } \left ( \textbf{C} | \textbf{X} \right )} \log p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) & = \bigtriangledown_{\phi } \sum_{\textbf{C}} p_{\phi } \left ( \textbf{C} | \textbf{X} \right ) \log p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) \\
& = \sum_{\textbf{C}} \log p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) \bigtriangledown_{\phi } p_{\phi } \left ( \textbf{C} | \textbf{X} \right )
\end{split}
\end{equation}
Helped by the log-derivative trick, we have:
\begin{equation}\label{Eq:Append_6}
\begin{split}
\sum_{\textbf{C}} \log p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) \bigtriangledown_{\phi } p_{\phi } \left ( \textbf{C} | \textbf{X} \right ) & = \sum_{\textbf{C}} \log p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) p_{\phi } \left ( \textbf{C} | \textbf{X} \right ) \bigtriangledown_{\phi } \log p_{\phi } \left ( \textbf{C} | \textbf{X} \right ) \\
& = \mathbb{E}_{\textbf{C}\sim p_{\phi } \left ( \textbf{C} | \textbf{X} \right )} \left [\log p\left ( \textbf{Y} | \textbf{C}, \textbf{X} \right ) \bigtriangledown_{\phi } \log p_{\phi } \left ( \textbf{C} | \textbf{X} \right ) \right ]
\end{split}
\end{equation}

==> Sections/Conclusion.tex <==
Our primary objective is to evaluate and tackle the challenge of compositional generalization in Data-to-Text Generation. To assess CG in DTG, we create a set of training splits using the WebNLG dataset. These splits are specifically designed to evaluate the model's capacity to be trained on examples with simple compositions comprising a very few predicates, and subsequently generalize to unseen compositions that consist of a larger number of predicates. 
In addition, we incorporate CG with few-shot learning and domain adaptation, resulting in four different testing scenarios with varying levels of difficulty. The experimental results reveal that the SoTA pre-trained model T5 struggles to generalize compositionally to unseen complex predicate compositions. To address this challenge, we introduce three clustering-based approaches that leverage the graph weights learned during training to decompose the unseen predicate compositions into familiar ones during testing. Our results demonstrate that our systems outperform the baseline T5 model by generating accurate text descriptions across all four testing scenarios.
In the future, we are enthusiastic about extending the concept of ``solving compositional generalization through learning to decompose'' to other text generation tasks. Additionally, we are open to integrating other CG-focused approaches, such as self-teaching, into our existing methods to further enhance their effectiveness.
